LLMic: Romanian Foundation Language Model

Recent advances in Large Language Models (LLMs) have demonstrated remarkable capabilities across various tasks with commercial models leading the way. While open models usually operate at a smaller scale, they maintain competitiveness through specialization and fine-tuning. However, a significant challenge persists: open models often underperform in low-resource languages due to limited representation in the training corpus. In this paper, we present LLMic, a bilingual foundation language model designed specifically for the Romanian Language. We document the complete process of pretraining a foundation model for a low-resource language, including corpus construction, architecture selection, and hyper-parameter optimization. Our evaluation demonstrates that LLMic can be specialized for tasks in the target language, achieving results comparable to other much larger open models. We show that fine-tuning LLMic for language translation after the initial pretraining phase outperforms existing solutions in English-to-Romanian translation tasks. This opens the path for efficient large-scale processing for the Romanian language community, using the much smaller LLMic model

==> 6-discussion.tex <==
\section{Related Work}

% Vorbeste Romaneste, Llama, EuroLLM, A Survey of Large Language Models for European
Fine-tuning has been used in practice for tuning models for a given language
language\cite{masala2024vorbecsti, garcia2024introducing}, but the results are
underwhelming compared to the languages that were representatively part of the
pretraining dataset.

% Ask Mihai: Why might to add a discussion about models learning, and how small models
% cannot learn multiple languages, and such we might need to pretrain them
A more resource-intensive approach is to pretrain the model on a corpus with
multiple languages\cite{dubey2024llama,ali2024survey}, but the performance is
often degraded for the less represented languages.


==> 7-conclusion.tex <==
\section{Conclusion}

